Secure Filtering against Spatio-Temporal False Data Attacks under Asynchronous Sampling

This paper addresses the secure state estimation problem for continuous linear time-invariant systems with non-periodic and asynchronous sampled measurements, where the sensors need to transmit not only measurements but also sampling time-stamps to the fusion center. This measurement and communication setup is well-suited for operating large-scale control systems and, at the same time, introduces new vulnerabilities that can be exploited by adversaries through (i) manipulation of measurements, (ii) manipulation of time-stamps, (iii) elimination of measurements, (iv) generation of completely new false measurements, or a combination of these attacks. To mitigate these attacks, we propose a decentralized estimation algorithm in which each sensor maintains its local state estimate asynchronously based on its measurements. The local states are synchronized through time prediction and fused after time-stamp alignment. In the absence of attacks, state estimates are proven to recover the optimal Kalman estimates by solving a weighted least square problem. In the presence of attacks, solving this weighted least square problem with the aid of $\ell_1$ regularization provides secure state estimates with uniformly bounded error under an observability redundancy assumption. The effectiveness of the proposed algorithm is demonstrated using a benchmark example of the IEEE 14-bus system.

==> deflatex3.tex <==

\def\Ac{{\mathcal A}}
\def\Abb{{\mathbb A}}
\def\Abf{{\mathbf A}}

\def\Bc{{\mathcal B}}
\def\Bbb{{\mathbb B}}
\def\Bbf{{\mathbf B}}

\def\Cc{{\mathcal C}}
\def\Cbb{{\mathbb C}}
\def\Cbf{{\mathbf C}}
\def\cc{{\mathcal c}}
\def\cfr{{\mathfrak c}}

\def\Dc{{\mathcal D}}
\def\Dbb{{\mathbb D}}
\def\Dbf{{\mathbf D}}

\def\Ec{{\mathcal E}}
\def\Ebb{{\mathbb E}}
\def\Ebf{{\mathbf E}}
\def\e{{\bf e}}

\def\Fc{{\mathcal F}}
\def\Fbb{{\mathbb F}}
\def\Fbf{{\mathbf F}}

\def\Gc{{\mathcal G}}
\def\Gbb{{\mathbb G}}
\def\Gbf{{\mathbf G}}

\def\Hc{{\mathcal H}}
\def\Hbb{{\mathbb H}}
\def\Hbf{{\mathbf H}}

\def\Ic{{\mathcal I}}
\def\Ibb{{\mathbb I}}
\def\Ibf{{\mathbf I}}

\def\Ii{{ {\mathbf e}   }}

\def\ei{{  {\mathbf e}_{\Psi} }}

\def\Jc{{\mathcal J}}
\def\Jbf{{\mathbf J}}
\def\Jbb{{\mathbb J}}

\def\Kc{{\mathcal K}}

\def\Lc{{\mathcal L}}
\def\Lbb{{\mathbb L}}
\def\Lrm{{\rm L}}
\def\Lbf{{\mathbf L}}
\def\Lfr{{\mathfrak L}}

\def\Mc{{\mathcal M}}
\def\Mbb{{\mathbb M}}
\def\Mbf{{\mathbf M}}

\def\Nc{{\mathcal N}}
\def\Nbb{{\mathbb N}}
\def\Nbf{{\mathbf N}}

\def\Oc{{\mathcal O}}
\def\Obb{{\mathbb O}}
\def\Obf{{\mathbf O}}

\def\Pc{{\mathcal P}}
\def\Pbb{{\mathbb P}}
\def\Pbf{{\mathbf P}}

\def\pfr{{\mathfrak p}}

\def\Qc{{\mathcal Q}}
\def\Qbb{{\mathbb Q}}
\def\Qbf{{\mathbf Q}}

\def\qfr{{\mathfrak q}}

\def\Rc{{\mathcal R}}
\def\Rbb{{\mathbb R}}
\def\Rbf{{\mathbf R}}
\def\Rfr{{\mathfrak R}}

\def\Sc{{\mathcal S}}
\def\Sbf{{\mathbf S}}
\def\Sbb{{\mathbb S}}

\def\Tc{{\mathcal T}}
\def\Tbb{{\mathbb T}}
\def\Tbf{{\mathbf T}}

\def\Uc{{\mathcal U}}
\def\Ubb{{\mathbb U}}
\def\Ubf{{\mathbf U}}

\def\Vc{{\mathcal V}}
\def\Vbb{{\mathbb V}}
\def\Vbf{{\mathbf V}}

\def\Wc{{\mathcal W}}
\def\Wbb{{\mathbb W}}
\def\Wbf{{\mathbf W}}

\def\Xc{{\mathcal X}}
\def\Xbb{{\mathbb X}}
\def\Xbf{{\mathbf X}}

\def\Yc{{\mathcal Y}}
\def\Ybb{{\mathbb Y}}
\def\Ybf{{\mathbf Y}}

\def\Zc{{\mathcal Z}}
\def\Zbb{{\mathbb Z}}
\def\Zbf{{\mathbf Z}}

\def\mat{{\mathbb M}}
\def\nat{{\mathbb N}}

\def\Th{{\Theta}}

\def\Xibf{{\bf \Xi}}

\def\th{{\theta}}

\def\pa{{\partial}}

\def\ep{{\epsilon}}

\def\om{{\omega}}
\def\Om{{\Omega}}

\def\Lmb{{\Lambda}}


\def\half{{\frac{1}{2}}}

\def\lam{{\lambda}}
\def\stm{{\setminus}}

\def\Sg{{\Sigma}}
\def\0{{\bf 0}}
\def\ker{{\rm ker}\,}
\def\dim{{\rm dim}\,}
\def\defe{\stackrel{\triangle}{=}}



%\newcommand{\st}{\stackrel{J}{\approx}}
\newcommand{\stt}{\stackrel{I}{\approx}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\btabular}{\begin{tabular}}
\newcommand{\etabular}{\end{tabular}}
\newcommand{\bcenter}{\begin{center}}
\newcommand{\ecenter}{\end{center}}
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\ba}{\left[ \begin{array}}
\newcommand{\ea}{\\ \end{array} \right]}
\newcommand{\bear}{\begin{array}}
\newcommand{\eear}{\\ \end{array}}

\newcommand{\tcr}{\textcolor{red}}
\newcommand{\tcb}{\textcolor{blue}}
\newcommand{\tcp}{\textcolor{purple}}
\newcommand{\ovl}{\overline}
%\newcommand{\ul}{\underline}
\newcommand{\wt}{\widetilde}

\newcommand{\br}{\breve}

\newcommand{\noi}{\noindent}
\newcommand{\non}{\nonumber}
\newcommand{\bb}{\cite}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\ran}{\rangle}
\newcommand{\lan}{\langle}
\newcommand{\Lolra}{\Longleftrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\btd}{\bigtriangledown}
\newcommand{\btu}{\bigtriangleup}
%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\newcommand{\ad}{{\rm \;\;\;\; and \;\;\;\;\;}}
\newcommand{\bs}{\boldsymbol}
%\newcommand*{\QED}{\hfill\ensuremath{\square}}%
\newcommand*{\QEDB}{\hfill\ensuremath{\blacksquare}}%
\newcommand*{\QET}{\hfill\ensuremath{\triangleleft}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\inpd}[1]{\left\langle#1\right\rangle}


%\def\Qced{{\ \vrule width 1.5mm height 1.5mm \smallskip}}



%\def\scalefig#1{\epsfxsize #1\textwidth}
%\def\scalefigy#1{\epsfysize #1\textwidth \epsfxsize 0.7\textwidth}

\newcounter{subequation}
\def\beasub{\addtocounter{equation}{+1}
\setcounter{subequation}{\value{equation}}
\setcounter{equation}{0}
\renewcommand{\theequation}{\arabic{subequation}\alph{equation}}
\begin{eqnarray}}
\def\eeasub{\end{eqnarray}
\setcounter{equation}{\value{subequation}}
\renewcommand{\theequation}{\arabic{equation}}}

%\newcommand{\over}{\overline}
\newcommand{\under}{\underline}
\newcommand{\mb}{\mathbf}
\newcommand{\tb}{\textbf}

%Tikz


%%  \usepackage[disable,colorinlistoftodos, textwidth=3cm, shadow]{todonotes} % disabled comments

\def\inf{\operatornamewithlimits{inf\vphantom{p}}}
\newtheorem{problem}{Problem}

\newcommand{\SCB}[1]{\todo[inline, color=gray!60]{\textbf{Sri:} #1}}

\newcommand{\AT}[1]{\todo[inline, color=orange!60]{\textbf{AT:} #1}}

\newcommand{\TN}[1]{\todo[inline, color=brown!60]{\textbf{TN:} #1}}


%upp

